Analysis of artifacts in EEG signals for building BCIs

Brain-Computer Interface (BCI) is an essential mechanism that interprets the human brain signal. It provides an assistive technology that enables persons with motor disabilities to communicate with the world and also empowers them to lead independent lives. The common BCI devices use Electroencephalography (EEG) electrical activity recorded from the scalp. EEG signals are noisy owing to the presence of many artifacts, namely, eye blink, head movement, and jaw movement. Such artifacts corrupt the EEG signal and make EEG analysis challenging. This issue is addressed by locating the artifacts and excluding the EEG segment from the analysis, which could lead to a loss of useful information. However, we propose a practical BCI that uses the artifacts which has a low signal to noise ratio. The objective of our work is to classify different types of artifacts, namely eye blink, head nod, head turn, and jaw movements in the EEG signal. The occurrence of the artifacts is first located in the EEG signal. The located artifacts are then classified using linear time and dynamic time warping techniques. The located artifacts can be used by a person with a motor disability to control a smartphone. A speech synthesis application that uses eyeblinks in a single channel EEG system and jaw clinches in four channels EEG system are developed. Word prediction models are used for word completion, thus reducing the number of artifacts required.

==> Chapter5.tex <==
As discussed in earlier chapters, Brain-computer interfaces (BCIs) are an exciting alternative to command a device. BCIs are often advantageous to people, who lost direction across all the muscles that oppositely could have been used as a medium of communication. For who would prefer to use BCIs, fortuitously, exist some consumer price (affordable) tools, which would enable to build a BCI on top of it. These EEG headsets can be employed for Electroencephalography (EEG) brain signal so that a machine can collect data. With that, people would reacquire a portion of their autonomy in mobility and communication. Through the BCI, they would succeed in the sense to command. It can comfortably be protracted to any electronic device. That would be a tremendous privilege and benefit.

In the last chapter, an economical way to apply the eyeblinks for building BCI was proposed. In this chapter, the work has been extended to for eyeblinks and jaw clenches for building a more effective BCI system in four electrodes EEG setup. Eye blinks and jaw clenches are predicted with the aid of time-warping techniques, as discussed in the chapter~\ref{chap:single}.

By developing BCI with an eyeblink and jaw clenches, a paralyzed subject may be equipped with communicating capabilities to the outer world. In this work, the eye blinks and jaw clenches are mapped to the various actions of the virtual keyboard. As we explained in the last chapter, we utilize a word completion models and text to speech synthesis (TTS) system to generate and output the synthesized speech concerning the word which subject intents to present.

\section{Experiment Setup} 

A four-channel muse EEG headset \citep{choosemuse} to acquire brain signal, with a wireless Bluetooth connection to transfer the EEG signal to the Android mobile phone is employed in this chapter. A brief preface about the muse EEG headset is presented in section \ref{sec:FEEG}.

\section{Preprocessing the signal}

The acquired EEG signal is preprocessed, as discussed in section \ref{sec:prep}.


\section{Artifacts prediction}

The crucial part of the building artifacts based BCI is to detect the presence of the artifacts in the EEG signal and predicting the type of the artifact. A simple yet powerful threshold technique is used to detect the artifacts and Dynamic time warping is employed to classify the type of the artifact. 

\subsection{Detection}
The Android application is equipped with a template for eyeblink and jaw clench. The threshold for the artifacts is estimated from template sequences as discussed in the section~\ref{sec:thres}. Whenever the realtime EEG crosses the threshold, we count the event as an appearance of the artifact. 

\subsection{Classification}
Once the artifact is detected, a chunk of EEG signal with the duration of 500~ms starting from the detection of the artifact is extracted. The extracted EEG signal is classified to obtain the type of artifact using DTW based classification technique, as mentioned in section~\ref{sec:dtw}. Based on the type of artifacts, the actions are mapped in the virtual keyboards, and it is discussed in the following sections.

\section{Virtual Prediction Keyboard}



\begin{figure*}[!ht]
\begin{minipage}[h]{1.2\linewidth}
 \centering
        \includegraphics[scale=0.6]{Images/Flowchart_chap5.png}
  \caption{Flow chart of Virtual Prediction Keyboard with Eye blinks and Jaw clenches}
  \label{Fig:chap5flow}
      \end{minipage}
\end{figure*}

The brief review about T9, ABC keyboards, their importance, developed T9, ABC virtual keyboards,  and its four regions, the navigation of each key, the operation of picking up the highlighted key with two consecutive eye blinks, character affixation, suggestion words mechanism, backspace mechanism, are discussed in sections~\ref{sec:T9} and \ref{sec:ABC}. 


As a contrast to the phrase region being highlighted for three seconds for two eye blinks, whenever the application encounter two consecutive jaw clenches, the words in the phrase region are sent to TTS, and the synthesized speech is presented. An illustrative flow chart for the mentioned process is shown in the figure~\ref{Fig:chap5flow}. This process repeats infinitely until the application exit.


\section{Speech synthesis}

The gathered words from the phrase region interact with Android Text To Speech (TTS) synthesizer API 4 \cite{android2018api} for speech generation as discussed in section \ref{sec:syn}


\section{Summary of the chapter}
In this chapter, a more reliable artifact-based BCI is developed for people with a speech disability. The proposed model employes eye blinks, and jaw clenches to produce a range of English words and that are synthesized to produce speech output with TTS. The chapter also evident that the artifacts based BCI can be incorporated in various EEG headset.

